Continual Deep Active Learning for Medical Imaging: Replay-Base Architecture for Context Adaptation

Deep Learning for medical imaging faces challenges in adapting and generalizing to new contexts. Additionally, it often lacks sufficient labeled data for specific tasks requiring significant annotation effort. Continual Learning (CL) tackles adaptability and generalizability by enabling lifelong learning from a data stream while mitigating forgetting of previously learned knowledge. Active Learning (AL) reduces the number of required annotations for effective training. This work explores both approaches (CAL) to develop a novel framework for robust medical image analysis. Based on the automatic recognition of shifts in image characteristics, Replay-Base Architecture for Context Adaptation (RBACA) employs a CL rehearsal method to continually learn from diverse contexts, and an AL component to select the most informative instances for annotation. A novel approach to evaluate CAL methods is established using a defined metric denominated IL-Score, which allows for the simultaneous assessment of transfer learning, forgetting, and final model performance. We show that RBACA works in domain and class-incremental learning scenarios, by assessing its IL-Score on the segmentation and diagnosis of cardiac images. The results show that RBACA outperforms a baseline framework without CAL, and a state-of-the-art CAL method across various memory sizes and annotation budgets. Our code is available in https://github.com/RuiDaniel/RBACA .

==> Images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}


==> sections/background_old.tex <==
\section{Background}

\label{stateofART}

The performance of DL techniques relies on both training and test sets being drawn from the same distribution, which is unlikely in the real world.
When such a shift in distribution occurs, one strategy is to rebuild models from scratch using newly collected training data, which can be unfeasible.

CL \citep{van2022three} involves adapting models to new contexts while maintaining performance on previously learned ones, without retraining from scratch at each new learning phase. There are 3 fundamental CL scenarios: Domain-Incremental Learning (Domain-IL), Task-Incremental Learning (Task-IL) and Class-Incremental Learning (Class-IL). 



Task-IL involves learning a set of clearly distinct contexts referred to as tasks. At all times task identity must be known. This approach allows training models with specific components or with distinct networks for each task. The main challenge lies in effectively sharing learned representations across tasks.
Domain-IL involves incrementally learning a particular task across various contexts, known as domains. At test time, domain identification is not required, as all domains share the same potential outputs.
Class-IL involves learning to discriminate among an increasing number of classes, which appear as contexts denominated episodes. A significant challenge is learning to discriminate between classes that have not been observed together, as different episodes can contain different classes.



CL strategies can be categorized into 3 families \citep{de2021continual}: memory-based, regularization-based, and parameter isolation methods. %However certain methods utilize techniques from multiple families.
Memory and replay mechanisms use storage to recall past contexts, combining new data with previous representations when learning a new context. These approaches face challenges related to memory requirements and privacy concerns, particularly in real-world applications like healthcare, where legislation often restricts long-term data storage \citep{masana2022class}.
These fall into 3 categories: rehearsal, pseudo-rehearsal, and constrained optimization. 
Rehearsal methods involve replayed stored samples. However, they may lead to overfitting on the replayed subset. In \cite{van2022three}, Experience Replay (ER) involves replayed data chosen uniformly at random from previous contexts. \cite{zheng2024selective} adapted ER to brain tumor segmentation. %On the other hand, Maximally Interferred Retrieval (MIR), presented in Aljundi \textit{et al.} \cite{DBLP:journals/corr/abs-1908-04742}, selects samples from previously learned contexts that are most likely to be forgotten.
The memory may also store latent representations. For instance, Incremental Classifier and Representation Learning (iCaRL) \citep{rebuffi2017icarl} learns strong classifiers and representations by storing templates closest to the feature mean of each class. %Another example is Brain-Inspired Replay (BI-R) \cite{van2020brain}, which replays generated representations at the latent feature level, which is applied for classifying retinal diseases in Verma \textit{et al.} \cite{verma2023privacy}.
Pseudo-rehearsal methods involve generating pseudo-samples using a generative model.
%Deep Generative Replay (DGR) \citep{shin2017continual} replays generated representations at the input level. 
Finally, constrained optimization allows for greater freedom in transferring knowledge between tasks. %Under Task-IL, Averaged Gradient Episodic Memory (A-GEM) \citep{chaudhry2019efficient} enforces that the loss on replayed data cannot increase during optimization of the loss on new data.



Regularization-based methods involve adding a regularization term to the loss, which penalizes changes to important parameters. %that represent previously learned contexts.
Data-focused techniques rely on functional regularization. When training on new contexts, they aim to retain input-output mapping at anchor points. Learning without Forgetting (LwF) \citep{li2017learning} uses current context inputs as anchors.
In contrast, prior-focused methods estimate parameter importance distribution. Elastic Weight Consolidation (EWC) \citep{kirkpatrick2017overcoming} quantifies it by utilizing the Fisher information matrix. EWC and LwF have been applied to classify optical diseases in \cite{verma2023privacy}.


Finally, parameter isolation employs distinct model parameters for each context. In fixed networks, the architecture remains static, with fixed context-specific components. %As a medical application, Bayasi \textit{et al.} \cite{bayasi2021culprit} approached skin lesion image classification using an architecture-based fixed partitioned network.
In contrast, dynamic architectures do not impose constraints on architecture size. They involve adding new units as new contexts emerge, updating both old and newly added parameters at different learning paces. %\citep{wang2017growing}. %In this scope, Growing a Brain \cite{wang2017growing} proposes several approaches for adding units to neural networks.

AL strives for high accuracy with a minimal number of annotations by selecting the most informative samples for labeling. The selection process involves a trained model from the labeled pool $L$. Newly labeled instances are added to $L$, and the model learns from them. %In contrast to serial selection, batch-mode selection allows querying instances in groups, which enhances labeling efficiency.
In \cite{settles1994active}, three AL scenarios are introduced: Membership Query Synthesis, Stream-Based Selective Sampling, and Pool-Based AL.
In the first one, the learner may request labels for any unlabeled instance within the input space, including queries it generates, which can lead to outliers.
In the second, the learner decides whether to label or discard each sequentially sampled unlabeled instance.
Finally, in Pool-Based AL, a pool of unlabeled data is evaluated to select the best query.



There are several methods for selecting the most informative samples to be labeled. Uncertainty Sampling \citep{lewis1995sequential} selects instances where the model is least confident about the labeling, with entropy \citep{shannon1948mathematical} commonly used as the uncertainty metric. %Biswas \textit{et al.} \cite{biswas2023active} tackle MRI detection using a framework based on this method.
Query-By-Committee (QBC) \citep{seung1992query} employs a committee of models, all trained on the current labeled set. The models vote on each instance's labeling, identifying the samples where they disagree the most. %\cite{grimova2019query} applied both QBC and Uncertainty Sampling to overnight polysomnography records classification.


In contrast, Expected Gradient Length (EGL) \citep{settles2007multiple} selects the instance whose labeling would result in the greatest gradient. However, as the true label is unknown, the gradient must be computed across potential labelings, which is computationally demanding.
Another method, Estimated Error Reduction, aims to minimize the generalization error. However, it requires incremental re-training for every potential labeling of each sample.


Batch selection aims to assemble the optimal query batch. Some strategies focus on informativeness, such as Bayesian Active Learning by Disagreement (BALD) \citep{houlsby2011bayesian}, applied by \cite{gal2017deep} for skin cancer diagnosis. However, these approaches may select a set of similar samples. To more accurately represent the input distribution, diversity-based approaches are used, and hybrid strategies consider both informativeness and diversity. BatchBALD \citep{kirsch2019batchbald} extends BALD by incorporating the correlation between batch data points.


DL can automatically learn and extract relevant features from annotated images. %, leveraging techniques such as CNNs. 
Deep AL \citep{ren2021survey} aims to minimize annotations and maintain DL capabilities. A DL model typically consists of feature extraction and task learning stages. Consequently, its uncertainty encompasses both stages' uncertainties. %Learning Loss for Active Learning (LLAL) \citep{yoo2019learning} leverages the output of multiple hidden layers as input for a loss prediction module, which guides the query strategy.
DL requires a substantial volume of labeled data for effective training. One strategy for expanding the labeled dataset involves assigning pseudo-labels to high-confidence samples, as in Cost-Effective Active Learning (CEAL) \citep{wang2016cost}. 


AL presents several challenges, such as a limited labeling budget and a lack of adaptability. Typically, models are retrained from scratch in each round, which is inefficient. Re-training and fine-tuning at each round is not viable due to forgetting. CL facilitates adaptation while minimizing forgetting. However, it requires all data to be labeled. These AL and CL disadvantages give rise to CAL, wherein the model progressively learns new information.


CAL methods have demonstrated the capability to surpass AL techniques, achieving noteworthy speedups. \cite{das2023continual} employs replay schemes involving model distillation and selects points based on diversity and uncertainty. %applied CL strategies to accelerate batch AL and facilitate the learning of new tasks. 
\cite{ayub2022few} present Few-Shot Continual Active Learning (FoCAL) for object classification, with a CL pseudo-rehearsal strategy and an AL uncertainty sampling.

Continual Active Learning for Scanner Adaptation (CASA), a CAL architecture developed by \cite{perkonigg2022continual}, is designed to process a continuous stream of images in a multi-scanner environment. It consists of a Domain-IL scenario of CL using a replay-based rehearsal method. An AL algorithm automatically detects shifts in image characteristics, selects examples for labeling within a limited labeling budget $\beta$, and adapts training accordingly. 


CASA comprises a Pseudo-Domain (PD) module, task module, outlier memory $O$, and rehearsal memory $M$. %, as illustrated in Fig. \ref{fig:CASA}. 
Initially, base training is conducted on a labeled dataset $L$ from a single scanner, where the task module is pre-trained on $L$, and $M$ is initialized with a random subset of $L$. The algorithm then observes the continuous data stream $S$ and detects domain shifts, forming Pseudo-Domains (PDs). %These PDs are used to assess whether training for a specific style is required and to diversify $M$. 
Samples belonging to newly detected PDs are labeled. PDs are clusters of samples with close style embeddings, which are computed through a fixed-style network. The PD module evaluates each sample, identifying the closest PD. If the distance to that PD is not below a threshold, the sample is added to $O$. Otherwise, the PD is known, and an AL method based on a performance metric (Perf) decides whether to route it to the oracle or discard it.


%The AL heuristic consists of selecting the samples corresponding to Pseudo-Domains (PDs) that are not yet complete and the entire newly detected PDs. Here, a Pseudo-Domain (PD) is considered complete if its samples have attained a certain performance metric threshold.

When $O$ receives a new item, a proximity evaluation between samples determines whether a new PD should be created and directed to the oracle. 
The oracle labels these instances and stores them in $M$, which is utilized for task module training. %, by sampling mini-batches and training through a step on each batch.
%$M$ preserves crucial examples from previous contexts, being balanced between 
$M$ has size $K_M$ and is balanced among existing PDs. %, with each of the $K_D$ PDs allowed to occupy up to $K_M/K_D$ elements. U
Upon the addition of a new PD, pruning is executed for each PD to maintain balance among them.
% a random subset of elements from all previous domains is flagged for deletion, maintaining only $K_M/K_D$ safeguarded elements per domain: there is a pruning procedure for each PD.
When a new element is stored in $M$ and its PD is fully occupied, it replaces the element with the closest embedding. %within the same PD.


There are several identified concerns associated with CASA's architecture. Its direct storage of samples poses a potential data privacy risk. Furthermore, the static nature of $K_M$ and $\beta$ is a limitation in dynamic situations. The early consumption of $\beta$ results in the non-representation of later PDs in $M$. With a small $K_M$, $M$ saturation may occur, compromising PDs representations, especially as the number of PDs increases. An excessively large $K_M$ may result in an imbalance in $M$ between PDs. Another concern is the use of Least Recently Used (LRU) pruning, which may remove crucial data. Moreover, regarding the AL method, once a PD reaches completion, it is no longer updated. However, this does not guarantee that there are no new highly informative samples.

Dataset pruning, without synthesizing representations, summarizes the dataset into a subset valuable for training by selecting which samples to retain and remove. There are various techniques available for this purpose. CASA uses LRU.
%There are distribution-based approaches that prioritize diversity and informativeness-based strategies that focus on choosing the most informative samples for the task.
In distribution-based approaches, clusters are formed with samples selected based on their proximity to each cluster's center. K-Means \citep{macqueen1967some} groups samples by assigning each point to the nearest cluster centroid, resulting in low computational complexity. However, it is sensitive to noise, does not account for variance, and requires the number of clusters in advance. In contrast, Gaussian Mixture Models (GMMs) \citep{reynolds2009gaussian} can handle clusters of arbitrary shapes by computing the probabilities of each point belonging to each cluster. Moreover, Density-Based Spatial Clustering of Applications with Noise (DBSCAN) \citep{ester1996density} provides a density-based approach to clustering that does not require specifying the number of clusters.
Informativeness-based techniques select the most informative samples using metrics such as uncertainty (Uncertainty Sampling) and gradient length (EGL).
Finally, there are hybrid approaches that balance diversity and informativeness.

% % \vspace{-0.5cm}
% \subsubsection{Privacy-preserving representations}
% \label{privacy-pres}


% In Wang \textit{et al.} \cite{wang2018dataset}, they developed an optimization algorithm for dataset distillation, facilitating faster model training due to fewer gradient descent steps. This algorithm aims to generate a small set of synthetic data samples that are not drawn from the real data distribution but can serve as training data to approximate a model trained on the original data. 
% This process involves minimizing the empirical error over the entire training data, as outlined in \eqref{DatasetDist1}, where $x_i$ represents a point from the training dataset, $\theta$ is the model parameterization, and $l(x_i, \theta)$ denotes the network's loss on $x_i$. 

% % \vspace{-0.4cm}
% \begin{equation}
%     \theta^* = \underset{\theta}{\arg\min} \frac{1}{N} \sum_{i=1}^{N} l(x_i, \theta)
%     \label{DatasetDist1}
% \end{equation}


% Asadi \textit{et al.} \cite{asadi2023prototype} introduced Prototype-Sample Relation Distillation (PRD) as a solution for strong private representation learning, demonstrating strong performance in both the Class-IL and Task-IL settings. The approach involves simultaneous learning of representations and class prototypes, ensuring the preservation of the relevance of previous class prototypes and their embedded similarities. Notably, real samples are not stored, and the method effectively employs relationship distillation alongside supervised contrastive learning. Samples are mapped to an embedding space where representations are learned through a supervised contrastive loss \cite{khosla2020supervised}, which integrates a contrastive loss along with a traditional supervised loss (such as Cross Entropy). The contrastive loss encourages the model to map similar examples close to each other in the feature space while pushing dissimilar examples apart.

% Furthermore, within the framework of PRD, class prototypes continually evolve in the same latent space, facilitating learning and prediction at any given point. The distillation loss plays a crucial role in constraining class prototypes to preserve their relative similarities compared to new task data. This preservation of the relative relationships among prototypes is achieved by minimizing changes in the softmax distribution over samples. For each prototype from prior tasks, the relative ordering of samples in the mini-batch is maintained, enabling representations to adapt to new classes while keeping the relevance of prototypes from previous classes.



% % \vspace{-0.5cm}
% \subsection{Conclusions}

% AL and CL enable DL algorithms to enhance their adaptability and generalization capabilities to novel image qualities and diverse contexts, fostering the transfer of knowledge across them. They provide an effective solution to the challenge of scarce annotations and help mitigate catastrophic forgetting.

% Despite the challenges and concerns inherent in both AL and CL methodologies, their fusion serves to alleviate these issues, presenting a viable framework for operating in a continuous stream featuring data from multiple contexts. CASA involves the automatic detection of context shifts in medical image acquisition characteristics, intending to strongly represent each context in a rehearsal memory. This memory is subsequently employed to train a task module, aiming to achieve optimal performance across all contexts.
% Nevertheless, various challenges emerge from the implementation of these approaches. % These challenges {\color{red} encompass data privacy issues, for which solutions may lie in the adoption of privacy-preserving representations.}
% The selection of rehearsal memory size and labeling budget poses considerations, as does determining which CL and AL methods can be integrated to enhance the effectiveness of representations. It is within the scope of these challenges that the work proposal is presented in chapter \ref{chap:proposta}.

